Bayesian hierarchical modelling for inferring genetic interactions in yeast

Quantitative Fitness Analysis (QFA) is a high-throughput experimental and computational methodology for measuring the growth of microbial populations. QFA screens can be used to compare the health of cell populations with and without a mutation in a query gene in order to infer genetic interaction strengths genome-wide, examining thousands of separate genotypes. We introduce Bayesian, hierarchical models of population growth rates and genetic interactions that better reflect QFA experimental design than current approaches. Our new approach models population dynamics and genetic interaction simultaneously, thereby avoiding passing information between models via a univariate fitness summary. Matching experimental structure more closely, Bayesian hierarchical approaches use data more efficiently and find new evidence for genes which interact with yeast telomeres within a published dataset.

==> models/Blocking.tex <==
\begin{align*}
l(K_l,K_{lm})=\prod_{m}^{M_{l}}\operatorname{N}(K_l;K_{lm},\frac{1}{e^{\tau^{K}_{l}}})=
\operatorname{N}(K_l;\mu^{*}_{K_l},{\sigma^{*2}_{K_l}})
\end{align*}
\begin{align*}
\mu^{*}_{K_l}=\sum_{m}^{M_{l}} \frac{K_{lm} }{ M_l}
\qquad 
{\sigma^{2}_{K_l}}=\frac{1 }{ M_{l}e^{\tau^{K}_{l}} }
\end{align*}
\begin{align*}
l(K,K_{l})=\prod_{l}^{L}\operatorname{N}(K;\mu^{*}_{K_l},\frac{1}{\frac{1}{e^{\sigma^{o2}_{K_l}}}+{\sigma^{*2}_{K_l}}})=
\operatorname{N}(K;\mu^{*}_{K},{\sigma^{*2}_{K_l}})
\end{align*}

\begin{align*}
\left.\mu^{*}_{K}=\sum_{L}^{l}\frac{\mu^{*}_{K_l}}{\frac{1}{e^{{\sigma^{o2}_{K}}}}+{\sigma^{*2}_{K_{l}}}} \middle/ \sum_{L}^{l}\frac{1}{\frac{1}{e^{{\sigma^{o2}_{K}}}}+{\sigma^{*2}_{K_{l}}}}  \right.
\qquad 
\left.{\sigma^{*2}_{K}}=1\middle/
\sum_{L}^{l}\frac{1}{\frac{1}{e^{{\sigma^{o2}_{K}}}}+{\sigma^{*2}_{K_{l}}}}\right.
\end{align*}
\begin{align*}
\pi(K|K_{lm})=\operatorname{N}(K;\frac{{\sigma^{*2}_{K}} K_{\mu}+\frac{1}{\eta^{p}_{K}}\mu^{*}_K}{{\sigma^{*2}_{K}}+\frac{1}{\eta^{p}_{K}}},\frac{{\sigma^{*2}_{K}} \frac{1}{\eta^{p}_{K}}}{{\sigma^{*2}_{K}}+\frac{1}{\eta^{p}_{K}}} )
\end{align*}
\begin{align*}
\pi(K_{l}|K,K_{lm})=\operatorname{N}(K_l;
\frac{
	{\sigma^{*2}_{K_{l}}} K + \frac{1}{ e^{ {\sigma^{o2}_{K}} } } \mu^{*}_{K_{l}}
	}{
	{\sigma^{*2}_{K_{l}}} + \frac{1}{ e^{ {\sigma^{o2}_{K}} } }
	}
,\frac{
	{\sigma^{*2}_{K_{l}}} \frac{1}{e^{{\sigma^{o2}_{K}}}}
	}{
	{\sigma^{*2}_{K_{l}}}+\frac{1}{e^{{\sigma^{o2}_{K}}}}} )
\end{align*}



==> sections/future.tex <==
\subsection{\label{Future Work}Future Work}
One of the long term goals of my work is to develop an R package that expands on the current QFA package used in \citet{QFA1}. The package will develop new methods and allow for analysis of the Lydall lab's QFA data sets. High throughput experiments in different areas of interest will also be able to make full use of the finished R package and perform QFA.   
Integrating my methods into the work of the Lydall lab would allow a more appropriate analysis of the many large datasets that are created by the lab as well as other genetic screens in yeast or other organisms. 
New methods for analysis of the QFA experiments should contribute to future papers of my own, the Lydall lab and others interested in performing QFA.

Deciding which model is the most biologically correct is a difficult task and future work includes comparing lists of known interactions with the new model results. 
By applying the new models developed to different datasets at different temperatures will allow us to further compare and contrast our new approaches.

Future models may be able to account for the fitness data at multiple temperatures simultaneously. 
The use of blocking within our MCMC may improve convergence time which is one of the biggest constraints of the new Bayesian methods. 

By improving the statistical methods used for QFA, statistical power can be increased. A smaller number of repeats can then be used to gain the same level of confidence. This means that instead of eight or more repeats per orf$\Delta$ strain, only four repeats per orf$\Delta$ strains may be necessary to carry out QFA. This may then improve the cost effectiveness for QFA while maintaining the same level of confidence.

After concluding our best model it should be possible for many relevant data sets with the problem of identifying genetic interaction to be make use of these new Bayesian models and improve their current inference.   
